Orchestra: Unsupervised Federated Learning via Globally Consistent Clustering

Federated learning is generally used in tasks where labels are readily available (e.g., next word prediction). Relaxing this constraint requires design of unsupervised learning techniques that can support desirable properties for federated training: robustness to statistical/systems heterogeneity, scalability with number of participants, and communication efficiency. Prior work on this topic has focused on directly extending centralized self-supervised learning techniques, which are not designed to have the properties listed above. To address this situation, we propose Orchestra, a novel unsupervised federated learning technique that exploits the federation's hierarchy to orchestrate a distributed clustering task and enforce a globally consistent partitioning of clients' data into discriminable clusters. We show the algorithmic pipeline in Orchestra guarantees good generalization performance under a linear probe, allowing it to outperform alternative techniques in a broad range of conditions, including variation in heterogeneity, number of clients, participation ratio, and local epochs.

==> backup.tex <==
\section{Symphony Behind Orchestra: Clusterability of Representations}
\label{sec:generalization}

% Spectral clustering~\cite{specloss} and its relation with SimSiam/BYOL~\cite{sslnocontrast}, 

% In a recent seminal work, Dennis et al.~\yrcite{fedcluster} show the task of clustering a predefined set of vectors thrives in federated settings: its sample complexity reduces with increased heterogeneity, it trivially scales to large clients, and the algorithm converges in just one round of communication. This motivates us to create an SSL framework that can exploit the many favorable properties of clustering in federated settings.


% \textbf{Theory of SSL:} Recently, substantial advances have been made towards demystifying SSL methods from the perspectives of learning theory~\cite{arora, specloss, sslgen}, information theory~\cite{multiviewssl}, causality~\cite{inversion, stylecontent}, and optimization~\cite{uniformity, sslnocontrast}. We extend the several tools proposed in these works to derive our results. These include two important assumptions, called ``expansion'' and ``separation'', and two important definitions, ``alignment'' and ``uniformity''. The notion of expansion and separation was originally proposed for manifolds by Balcan et al.~\yrcite{expansion}, recently verified empirically by Wei et al.~\yrcite{selftraining}, and converted to graph connectivity properties by HaoChen et al.~\yrcite{specloss}. Specifically, the authors assume that there exists a latent graph instantiating the data distribution such that the neighborhood of any low probability set of connected nodes has a higher probability than the set itself. Here a node represents a sample and edges represent joint probability of occurrence of two samples. Under expansion, any given community of nodes on the latent graph is guaranteed to be sufficiently well connected such that if a node with high enough probability is assigned a label, then via a loss promoting consistency to input perturbations, the label will propagate throughout the community. If communities are assumed to be well separated, these labels will have higher diffusion within the same community than between different communities. This induces sets of abstract classes with semantically related nodes (e.g., community of dogs). Using standard pairwise clustering tools, one can compute node representations that enable discrimination between these communities and, if a sufficiently expressive parametric model (e.g., a neural network) is trained to match these representations, it can be guaranteed the model will have small generalization error on unseen data. \ak{I'm wondering if this graph-based explanation would be easy to understand for SSL+CV folks. Are there alternate explanations that might be easier and more accessible for a typical CV reviewer?} The approach outlined above was recently used by HaoChen et al.~\yrcite{specloss} to design \emph{SpecLoss}, an SSL technique with provable generalization guarantees. We will take a similar approach to develop Orchestra, but will deviate in the clustering methodology. Specifically, since pairwise clustering requires computation of representation similarity between different datapoints, it is not amenable to use in decentralized, privacy-sensitive settings. We will circumvent this issue by designing a partition-based, federated clustering framework that first computes centroids capable of partitioning the federation's data into discriminable clusters and then asks clients to allocate their data into these clusters.

\begin{figure}
\centering
\begin{subfigure}{0.48\columnwidth}
  \centering
  \centerline{\includegraphics[width=\columnwidth]{figures/exptt_orchestra_comms_c10.pdf}}
\end{subfigure}%
\begin{subfigure}{0.48\columnwidth}
  \centering
  \centerline{\includegraphics[width=\columnwidth]{figures/exptt_orchestra_comms_c100.pdf}}
\end{subfigure}
\vspace{-2mm}
\caption{\label{fig:orchestra_comms} \textbf{Heterogeneity improves communication efficiency} for Orchestra on CIFAR-10 (left) and CIFAR-100 (right), i.e., Orchestra thoroughly exploits heterogeneity to maximize efficiency.}
\vspace{-10pt}
\end{figure}


\textbf{Effect of Heterogeneity on Communication Efficiency.} Our theoretical result indicates and empirical results corroborate the expectation that Orchestra thrives under heterogeneity. We provide another demonstration of this result in \autoref{fig:orchestra_comms}, where we show the progress of kNN accuracy as a model is trained using Orchestra. We find that not only does heterogeneity help Orchestra improve performance, it can in fact improve its speed of optimization. Overall, we see Orchestra is highly amenable to use with practical constraints of FL.


% We further show below that one can guarantee similarity-based cluster assignment will work well locally. That is, even though we only share the local centroids, we can simply compute the similarity of a sample's representation with the global centroids to determine which cluster it belongs to.
% \begin{claim}
% \label{prop:assigns}
% Let $d(x, \mu_{1}, \mu_{2}) = \norm{x - \mu_{2}}^{2} - \norm{x - \mu_{1}}^{2}$. Compute $\mu^{G} = \mathcal{C}(\mu^{L})$, where $\mu^{L} = \{\mathcal{C}(R_{X^{k)}}): k \in [K]\}$ denotes set of local centroids. Denote sample $x$'s assigned local cluster as $l$, whose centroid $\mu_{l}$ is assigned to cluster $g_i$. Then, for all $j \in [G] - \{i\}$, we have
% \begin{equation}
% % \text{P}(d(x, \mu_{g_i}, \mu_{g_j}) > t) \leq \mathcal{O}(e^{-d(\mu_l, \mu_{g_i}, \mu_{g_j})}).
% \mathbb{E}_{x\in l}[d(x, \mu_{g_i}, \mu_{g_j})] = d(\mu_{l}, \mu_{g_i}, \mu_{g_j}).
% \end{equation}
% \end{claim}
% The result above shows that, on average, if a local centroid is assigned to a global cluster, its corresponding samples will have high similarity with that cluster's centroid too. This implies one can use similarity-based assignment methods to determine which cluster a sample is assigned to.

